IRR: Image Review Ranking Framework for Evaluating Vision-Language Models

Large-scale Vision-Language Models (LVLMs) process both images and text, excelling in multimodal tasks such as image captioning and description generation. However, while these models excel at generating factual content, their ability to generate and evaluate texts reflecting perspectives on the same image, depending on the context, has not been sufficiently explored. To address this, we propose IRR: Image Review Rank, a novel evaluation framework designed to assess critic review texts from multiple perspectives. IRR evaluates LVLMs by measuring how closely their judgments align with human interpretations. We validate it using a dataset of images from 15 categories, each with five critic review texts and annotated rankings in both English and Japanese, totaling over 2,000 data instances. The datasets are available at https://hf.co/datasets/naist-nlp/Wiki-ImageReview1.0. Our results indicate that, although LVLMs exhibited consistent performance across languages, their correlation with human annotations was insufficient, highlighting the need for further advancements. These findings highlight the limitations of current evaluation methods and the need for approaches that better capture human reasoning in Vision & Language tasks.

==> fig/fig2.tex <==
\begin{figure}[]
\centering
\includegraphics[width=0.98\columnwidth]{image/figure2.pdf}
\caption{An evaluation metric using rank correlation analysis with an image and five review texts.}
\label{fig:rank_corre}
\end{figure}





==> table/GPT-4V_result.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{rr}
    \toprule
     %& {\bf {\small mPLUG-Owl}} & {\bf {\small mPLUG-Owl2}} & {\bf {\small Qwen-VL}} \\ 
     & GPT-4V\\ 
    \midrule
    EN & 0.399 \\
    JA & 0.506 \\

    \bottomrule
    \end{tabular}
    \caption{Rank correlations between GPT-4V and top-correlated annotators.}
    \label{tab:GPT_result}
\end{table}

==> table/learning_data.tex <==
% Adjust caption settings
\captionsetup[longtable]{position=bottom}

{\scriptsize % 表全体のフォントサイズを小さくする
\centering
\begin{longtable}{llcccc}
    \toprule
    \textbf{Data Type} & \textbf{Data Name} & \textbf{mPlug-owl} & \textbf{Qwen-VL-Chat} & \textbf{LLava-v-1.5} & \textbf{InstructBLIP} \\
    \midrule
    \endfirsthead

    \toprule
    \textbf{Data Type} & \textbf{Data Name} & \textbf{mPLUG-Owl2} & \textbf{Qwen-VL-Chat} & \textbf{LLava-v-1.5} & \textbf{InstructBLIP} \\
    \midrule
    \endhead

    \midrule
    \endfoot

    \bottomrule
    \endlastfoot

    Text & ShareGPT \cite{chen2023sharegpt4v} & \CheckmarkBold &  & \CheckmarkBold &  \\
    & SlimOrca \cite{mukherjee2023orca} & \CheckmarkBold &  &  &  \\
    & In-house Data &  & \CheckmarkBold &  &  \\
    Dialogue & LLaVA \cite{liu2023llava} & \CheckmarkBold &  & \CheckmarkBold &  \\
    Caption & COCO \cite{Lin2014MicrosoftCC} & \CheckmarkBold & \CheckmarkBold &  & \CheckmarkBold \\
    & TextCaps \cite{sidorov2020textcaps}& \CheckmarkBold &  & \CheckmarkBold & \CheckmarkBold \\
    & SBU \cite{inproceedings} &  & \CheckmarkBold &  &  \\
    & Coyo \cite{kakaobrain2022coyo-700m} &  & \CheckmarkBold &  &  \\
    & DataComp \cite{datacomp} &  & \CheckmarkBold &  &  \\
    & CC12M \& 3M \cite{changpinyo2021cc12m} &  & \CheckmarkBold &  &  \\
    & LAION-en \cite{schuhmann2022laion5b} \& zh &  & \CheckmarkBold &  &  \\
    VQA & VQAv2 & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold \\
    & GQA \cite{8953451} & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold \\
    & OKVQA \cite{8953725} & \CheckmarkBold &  & \CheckmarkBold & \CheckmarkBold \\
    & OCRVQA \cite{8978122} & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold \\
    & A-OKVQA \cite{inbook}& \CheckmarkBold &  & \CheckmarkBold & \CheckmarkBold \\
    & DVQA \cite{kafle2018dvqa} &  & \CheckmarkBold &  &  \\
    & TextVQA \cite{Singh2019TowardsVM}&  & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold \\
    & ChartQA \cite{masry-etal-2022-chartqa} &  & \CheckmarkBold &  &  \\
    & A12D &  & \CheckmarkBold &  &  \\
    Grounding² & GRIT \cite{Kosmos2} &  & \CheckmarkBold &  &  \\
    Ref Grounding & GRIT &  & \CheckmarkBold &  &  \\
    & VisualGenome \cite{Krishna2016VisualGC} &  & \CheckmarkBold & \CheckmarkBold &  \\
    & RefCOCO \cite{article}&  & \CheckmarkBold & \CheckmarkBold &  \\
    & RefCOCO+ \cite{article}&  & \CheckmarkBold & \CheckmarkBold &  \\
    & RefCOCOg &  & \CheckmarkBold & \CheckmarkBold &  \\
    OCR & SynthDoG-en \cite{kim2022donut} \& zh &  & \CheckmarkBold &  &  \\
    & Common Crawl pdf \& HTML &  & \CheckmarkBold &  &  \\
    Image Captioning & Web CapFilt \cite{https://doi.org/10.48550/arxiv.2201.12086}&  &  &  & \CheckmarkBold \\
    & NoCaps &  &  &  & \CheckmarkBold \\
    & Flickr30K \cite{deeplake}&  &  &  & \CheckmarkBold \\
    Visual Spatial Reasoning & IconQA \cite{lu2021iconqa}&  &  &  & \CheckmarkBold \\
    Visual Dialog & Visual Dialog &  &  &  & \CheckmarkBold \\
    Video Question Answering & MSVD-QA \cite{xu2017video}&  &  &  & \CheckmarkBold \\
    & MSRVTT-QA &  &  &  & \CheckmarkBold \\
    & iVQA \cite{8578996}&  &  &  & \CheckmarkBold \\
    Image Classification & VizWiz \cite{Gurari2018VizWizGC}&  &  &  & \CheckmarkBold \\
    Knowledge-Grounded Image QA & ScienceQA \cite{lu2022learn}&  &  &  & \CheckmarkBold \\
    \caption{Details of training datasets.}
    \label{tab:training_datasets} \\
\end{longtable}

} % 終了: \small


==> table/prompt_ja.tex <==
\begin{table}[h]
    \centering
    % \caption{鑑賞文の生成に用いたprompt}
    \textbf{鑑賞文の生成に用いたprompt}
    \label{tab:hogehoge}
    \begin{tabular}{|p{0.9\linewidth}|}
        \hline
        画像の良い点と改善可能な点について記述した異なる5つの鑑賞文を下記の制約に従って記述してください。\\
        1. 各鑑賞文の内容が異なっている。\\
        2. 各鑑賞文の長さがほぼ同じである。\\
        3. 鑑賞文中に箇条書きを含めない。\\
        4. 鑑賞文は「客観的で整合性が高い」、「主観的だが整合性が高い」、「客観的だが整合性が低い」、「主観的で整合性が低い」、「主観的で誤りを含む」ものをこの順序で5つ記述する。\\
        5. 各鑑賞文が画像の良い点と改善可能な点について記述している。\\
        6. 画像に改善可能な点が存在しない場合は鑑賞文中にそのことを明示する。\\ \hline
    \end{tabular}
\end{table}

==> table/rlhf.tex <==
\begin{screen}
Please describe a review text about the good points and room for improvement of the image
    
\end{screen}

